FineFake: A Knowledge-Enriched Dataset for Fine-Grained Multi-Domain Fake News Detection

Existing benchmarks for fake news detection have significantly contributed to the advancement of models in assessing the authenticity of news content. However, these benchmarks typically focus solely on news pertaining to a single semantic topic or originating from a single platform, thereby failing to capture the diversity of multi-domain news in real scenarios. In order to understand fake news across various domains, the external knowledge and fine-grained annotations are indispensable to provide precise evidence and uncover the diverse underlying strategies for fabrication, which are also ignored by existing benchmarks. To address this gap, we introduce a novel multi-domain knowledge-enhanced benchmark with fine-grained annotations, named \textbf{FineFake}. FineFake encompasses 16,909 data samples spanning six semantic topics and eight platforms. Each news item is enriched with multi-modal content, potential social context, semi-manually verified common knowledge, and fine-grained annotations that surpass conventional binary labels. Furthermore, we formulate three challenging tasks based on FineFake and propose a knowledge-enhanced domain adaptation network. Extensive experiments are conducted on FineFake under various scenarios, providing accurate and reliable benchmarks for future endeavors. The entire FineFake project is publicly accessible as an open-source repository at \url{https://github.com/Accuser907/FineFake}.

==> Table/MVAE_ex.tex <==
% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%   \centering
%   \caption{Add caption}
%     \begin{tabular}{l|r|r|r}
%     \toprule
%     Source/Target & \multicolumn{1}{l|}{Stream Media} & \multicolumn{1}{l|}{Official News} & \multicolumn{1}{l}{Fact-check Web} \\
%     \midrule
%     Stream Media & 100   & 100   & 100 \\
%     \midrule
%     Official News & 100   & 100   & 100 \\
%     \midrule
%     Fact-check Web & 100   & 100   & 100 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table}%

% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%   \centering
%   \caption{Add caption}
%     \begin{tabular}{l|r|r|r}
%     \toprule
%     Source/Target & \multicolumn{1}{l|}{Politics} & \multicolumn{1}{l|}{Entertainment} & \multicolumn{1}{l}{Conflict} \\
%     \midrule
%     Politics & 100   & 100   & 100 \\
%     \midrule
%     Entertainment & 100   & 100   & 100 \\
%     \midrule
%     Conflict & 100   & 100   & 100 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table}%

\begin{table}[t]
    \centering
    \begin{minipage}[b]{0.45\linewidth}
    \centering
    \label{cross-platform}
    \begin{tabular}{l|r|r|r}
    \toprule
    S/T & \multicolumn{1}{l|}{Str. } & \multicolumn{1}{l|}{Offi.} & \multicolumn{1}{l}{F-C} \\
    \midrule
    Str. & 0.793   & 0.283   & 0.618 \\
    \midrule
    Offi. & 0.327   & 0.810   & 0.333 \\
    \midrule
    F-C & 0.628   & 0.280   & 0.657 \\
    \bottomrule
    \end{tabular}%
    \caption{Cross-platform experiment, accuracy is the metric.
    Str: Stream Media; Offi:Official Media; F-C: Fact-check websites}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.45\linewidth}
    \centering
    \label{cross-topic}
    \begin{tabular}{l|r|r|r}
    \toprule
    S/T & \multicolumn{1}{l|}{Pol.} & \multicolumn{1}{l|}{Ent.} & \multicolumn{1}{l}{Con.} \\
    \midrule
    Pol. & 0.675   & 0.670   & 0.592 \\
    \midrule
    Ent. & 0.614   & 0.742   & 0.646 \\
    \midrule
    Con. & 0.627   & 0.545   & 0.659 \\
    \bottomrule
    \end{tabular}%
    \caption{Cross-topic experiment, accuracy is the metric. Pol : Politics topic; Ent
    : Entertainment topic;
     Con : Conflict topic}
    \end{minipage}
    \label{mvae-cross}
    \vspace{-0.5cm}
\end{table}


==> Table/beifen.tex <==
Task 2:
% 格式按照Acc,BA,F1去做
        Acc BA F1 Acc BA F1 Acc BA F1
EANN    /  /  /  0.763 0.531 0.731 0.621 0.545 0.607
MDFEND  / /  /  0.782 0.514 0.727 0.615 0.554 0.609
M3FEND  / /  /  0.763 0.536 0.763 0.661 0.538 0.604
CANMD  /  /  / 0.802 0.498 0.890 0.549 0.575 0.492

        Acc BA F1 Acc BA F1 Acc BA F1
EANN   0.412 0.425 0.427  / / / 0.401 0.485 0.379
MDFEND 0.679 0.671  0.686 / / / 0.477 0.532 0.479
M3FEND 0.566 0.604 0.576 / / / 0.411 0.504 0.383
CANMD 0.521 0.557 0.478 / / / 0.487 0.508 0.425

        Acc BA F1 Acc BA F1 Acc BA F1
EANN  0.721 0.693 0.723    0.804 0.500 0.718    / / /
MDFEND 0.703 0.698 0.710    0.784 0.497 0.715   / / / 
M3FEND  0.721 0.607 0.679    0.688 0.509 0.690 / / /
CANMD 0.669 0.622 0.491       0.678 0.480 0.801/ / /


Task 1：
        Acc BA F1 Acc BA F1 
EANN   0.924 0.852 0.921 0.714 0.634 0.678
MDFEND  0.920 0.869 0.919 0.697 0.667 0.695
M3FEND  0.912 0.847 0.910 0.649 0.676 0.655
CANMD  0.927 0.847 0.923 0.697 0.664 0.694

        Acc BA F1 Acc BA F1 
EANN  0.945 0.512 0.923 0.838 0.560 0.804
MDFEND 0.948 0.526 0.927 0.847 0.513  0.783
M3FEND 0.947 0.500 0.921 0.836 0.547  0.798
CANMD 0.947 0.500 0.921  0.823 0.522  0.782

        Acc BA F1 Acc BA F1 Acc BA F1
EANN  0.653 0.597 0.631 0.654 0.598 0.631
MDFEND 0.661 0.632 0.657 0.629 0.603 0.627
M3FEND  0.632 0.624 0.636 0.616 0.514 0.514
CANMD  0.691 0.664 0.688  0.635 0.624 0.638

Task 3:
        Acc BA F1 Acc BA F1 Acc BA F1
EANN    /  /  /  0.825 0.541 0.794 0.710 0.591 0.689
MDFEND  / /  /  0.802 0.559 0.789 0.697 0.586 0.681
M3FEND  / /  /  0.840 0.550 0.804 0.706 0.563 0.671
CANMD  /  /  / 0.791 0.486 0.882 0.653 0.598 0.434

        Acc BA F1 Acc BA F1 Acc BA F1
EANN   0.381 0.396 0.423  / / / 0.326 0.482 0.265
MDFEND 0.746 0.669  0.753 / / / 0.509 0.523 0.533
M3FEND 0.666 0.620 0.687 / / / 0.483 0.537 0.501
CANMD 0.318 0.511 0.367 / / / 0.290 0.504 0.443

        Acc BA F1 Acc BA F1 Acc BA F1
EANN  0.771 0.657 0.767    0.839 0.498 0.776    / / /
MDFEND 0.772 0.664 0.769    0.828 0.500 0.776  / / / 
M3FEND  0.753 0.675 0.758    0.849 0.500 0.779 / / /
CANMD 0.786 0.596 0.344       0.769 0.485 0.868/ / /

new task3 best
        Acc BA F1 Acc BA F1 Acc BA F1
EANN    /  /  /   0.770 0.507 0.721 0.647 0.526 0.592
MDFEND  / /  /  0.799 0.501 0.719 0.635 0.544 0.609
M3FEND  / /  /  0.788 0.506 0.723 0.599 0.526 0.588
CANMD  /  /  /  0.506 0.487 0.628 0.486 0.504 0.420

        Acc BA F1 Acc BA F1 Acc BA F1
EANN    0.687 0.710 0.696 / / /  0.621 0.540 0.603
MDFEND 0.691 0.606 0.670/ / / 0.638 0.536 0.603
M3FEND  0.665 0.613 0.662/ / / 0.642 0.520 0.585
CANMD  0.331 0.500 0.497/ / /  0.334 0.500 0.500

        Acc BA F1 Acc BA F1 Acc BA F1
EANN     / / / 0.686 0.697 0.695 0.780 0.509 0.724
MDFEND  / / / 0.728 0.698 0.730 0.784 0.506 0.722
M3FEND   / / /0.734 0.684 0.729 0.804 0.500 0.717
CANMD / / / 0.716 0.658 0.531 0.702 0.511 0.816

new task3 normal
        Acc BA F1 Acc BA F1 Acc BA F1
EANN    /  /  /  0.666 0.510 0.678 0.568 0.493 0.557
MDFEND  / /  /  0.741  0.494  0.705 0.581 0.523 0.578
M3FEND  / /  /  0.788 0.506 0.723 0.667 0.502 0.538
CANMD  /  /  /  0.506 0.487 0.628 0.486 0.504 0.420

        Acc BA F1 Acc BA F1 Acc BA F1
EANN   0.673 0.629 0.672/ / / 0.423 0.514 0.398
MDFEND 0.619 0.695 0.620/ / / 0.551 0.513 0.558
M3FEND  0.537 0.625 0.527/ / / 0.556 0.533 0.566
CANMD 0.331 0.500 0.497/ / /  0.334 0.500 0.500

        Acc BA F1 Acc BA F1 Acc BA F1
EANN   / / / 0.651 0.566 0.631 0.711 0.550 0.714
MDFEND   / / / 0.685 0.611 0.671 0.757 0.506 0.717
M3FEND  / / /0.665 0.606 0.659 0.619 0.537 0.652
CANMD / / /0.634 0.60 0.476 0.685 0.505 0.804

acc pre rec f1
MVAE   fact_check_p_train fact_check_p_test
0.657 0.558 0.520 0.481
MVAE   fact_check_e fact_check_p_test
0.595 0.446 0.471 0.438
MVAE   official_p fact_check_p_test
0.333 0.166 0.5 0.250

Pol
0.793 0.283 0.618
0.327 0.810 0.333
0.628 0.280 0.657


fact_check
0.657 0.611 0.588
0.624 0.646 0.555
0.653 0.553 0.616

==> Table/fine-grained_classification.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}
% \begin{table}[htbp]
  \centering
%   \renewcommand{\arraystretch}{1}
%   \setlength\tabcolsep{5.5pt}
%   \setlength{\abovecaptionskip}{-0.1cm}
% \setlength{\belowcaptionskip}{0.1cm} 
  \caption{Fine-grained classification results, best results are in \textbf{bold} and second ones are \underline{underlined}.}
    \begin{tabular}{l|cccc}
    \toprule
    \multicolumn{1}{l|}{\multirow{2}[1]{*}{Methods}} & \multicolumn{1}{c}{\multirow{2}[1]{*}{Acc}} & \multicolumn{1}{c}{\multirow{2}[1]{*}{Precision}} & \multicolumn{1}{c}{\multirow{2}[1]{*}{Recall}} & \multicolumn{1}{c}{\multirow{2}[1]{*}{F1-score}} \\
          &       &       &       &  \\
    \midrule
    SAFE  &0.642       &0.536       &0.611       &0.571  \\
    MVAE  &0.588       &0.543       &0.592       &0.566  \\
    BERT  &0.763       &0.759       &0.780       &0.769  \\
    CLIP  &0.772       &0.760       &\textbf{0.807}       &0.787  \\
    % VILT &       &       &       &  \\
    MDFEND &\underline{0.791}       &\underline{0.804}       &0.783       &\underline{0.793}  \\
    M3FEND &\textbf{0.794}       &\textbf{0.818}       &\underline{0.806}       &\textbf{0.811}  \\
    \bottomrule
    \end{tabular}%
  \label{tab:fine-grained}%
% \end{table}%
 \vspace{-0.4cm}
\end{table}

% \begin{wraptable}{r}{4.3cm}
% 	\centering
% 	\begin{tabular}{lrrr}
% 	%.....
% 	\end{tabular}
% \end{wraptable}

==> Table/multidomain.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[!htbp]
  \centering
  \renewcommand{\arraystretch}{1} % 行高
  \setlength{\abovecaptionskip}{-0.1cm} 
% \setlength{\belowcaptionskip}{0cm} 
  \caption{Multi-domain adaptation results, best results are in \textbf{bold} and second ones are \underline{underlined}.}
    \begin{tabular}{l|cccc|cccc}
    \toprule
    \multicolumn{1}{l|}{\multirow{2}[3]{*}{Methods}} & \multicolumn{4}{c|}{Sports} & \multicolumn{4}{c}{Technology} \\
\cmidrule{2-9}          & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{Pre} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{l|}{F1-score} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{Pre} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1-score} \\
    \midrule
    SAFE  &0.578       &0.588       &0.540       &0.563       &0.604       &0.598       &0.637       &0.617  \\
    MVAE  &0.571       &0.558       &0.682       &0.614       &0.615       &0.465       &0.657       &0.544  \\
    BERT  & 0.852      & \textbf{0.869}      & \underline{0.885}      & \underline{0.877}      & \underline{0.816}      & \textbf{0.878}      & \underline{0.826}      & \underline{0.851} \\
    CLIP  & \textbf{0.862}      & 0.839      & \textbf{0.947}      & \textbf{0.890}      & 0.799      & \underline{0.860}      & 0.818      & 0.839 \\
    MDFEND       &0.797       &\underline{0.856}       &0.797       &0.825  & \textbf{0.844}       & 0.836       &\textbf{0.874}       &\textbf{0.855} \\
    M3FEND & \underline{0.853}       &0.853     & 0.852       &0.852      &0.755       &0.751       &0.686       &0.717  \\
    \bottomrule
    \end{tabular}%
    \vspace{-0.4cm}
  \label{tab:domain adaptation}%
\end{table*}%

